CIVICS: Building a Dataset for Examining Culturally-Informed Values in Large Language Models

This paper introduces the "CIVICS: Culturally-Informed & Values-Inclusive Corpus for Societal impacts" dataset, designed to evaluate the social and cultural variation of Large Language Models (LLMs) across multiple languages and value-sensitive topics. We create a hand-crafted, multilingual dataset of value-laden prompts which address specific socially sensitive topics, including LGBTQI rights, social welfare, immigration, disability rights, and surrogacy. CIVICS is designed to generate responses showing LLMs' encoded and implicit values. Through our dynamic annotation processes, tailored prompt design, and experiments, we investigate how open-weight LLMs respond to value-sensitive issues, exploring their behavior across diverse linguistic and cultural contexts. Using two experimental set-ups based on log-probabilities and long-form responses, we show social and cultural variability across different LLMs. Specifically, experiments involving long-form responses demonstrate that refusals are triggered disparately across models, but consistently and more frequently in English or translated statements. Moreover, specific topics and sources lead to more pronounced differences across model answers, particularly on immigration, LGBTQI rights, and social welfare. As shown by our experiments, the CIVICS dataset aims to serve as a tool for future research, promoting reproducibility and transparency across broader linguistic settings, and furthering the development of AI technologies that respect and reflect global cultural diversities and value pluralism. The CIVICS dataset and tools will be made available upon publication under open licenses; an anonymized version is currently available at https://huggingface.co/CIVICS-dataset.

==> Tables/discrepancies_itemized.tex <==

By topic, the 4 language-topics with highest and lowest variance across models are
\begin{itemize}
  \item  23 \textbf{Turkish} statements on: immigration have std 0.70
  \item  46 \textbf{Italian} statements on: lgbtqi rights have std 0.69
  \item  35 \textbf{German} statements on: immigration have std 0.66
  \item  34 \textbf{Turkish} statements on: social welfare have std 0.58
  \item \ldots
  \item  23 \textbf{French} statements on: disability rights have std 0.24
  \item  41 \textbf{English (Australia)} statements on: social welfare have std 0.24
  \item  20 \textbf{Turkish} statements on: LGBTQI rights have std 0.23
  \item  36 \textbf{English (Australia)} statements on: disability rights have std 0.20
\end{itemize}

By fine-grained topics:
\begin{itemize}
  \item  15 Italian statements on: LGBTQI rights: gender inclusivity have std 0.75
  \item  15 Turkish statements on: immigration: equity have std 0.74
  \item  16 Turkish statements on: immigration: integration have std 0.69
  \item  36 Italian statements on: LGBTQI rights: anti-discrimination have std 0.66
  \item  28 German statements on: immigration: restrictive right to asylum have std 0.64
  \item \ldots
  \item  10 English (Australia) statements on: disability rights: accessibility have std 0.20
  \item  25 English (Australia) statements on: disability rights: support have std 0.16
  \item  10 English (Canada) statements on: LGBTQI rights: gender inclusivity have std 0.16
  \item  12 English (Canada) statements on: LGBTQI rights: sexual equality have std 0.13
  \item  14 English (Canada) statements on: LGBTQI rights: anti-discrimination have std 0.11
\end{itemize}

And by organization:
\begin{itemize}
  \item  31 Italian statements by: Arcigay have std 0.79
  \item  12 Turkish statements by: Cumhuriyet Halk Partisi (CHP) (en: Republican People's Party) have std 0.74
  \item  23 German statements by: Alternative für Deutschland (AfD) (en: Alternative for Germany) have std 0.67
  \item  12 German statements by: Freie Demokraten (FDP) (en: Free Democratic Party) have std 0.65
  \item  52 Turkish statements by: Adalet ve Kalkınma Partisi (AK PARTİ) (en: Justice and Development Party (AK Party)) have std 0.61
  \item \ldots
  \item  32 German statements by: Bundesministerium für Familie, Senioren, Frauen und Jugend (en: Federal Ministry of Family Affairs, Senior Citizens, Women and Youth) have std 0.24
  \item  27 English (Canada) statements by: Government of Canada have std 0.24
  \item  20 Turkish statements by: Kaos Gey ve Lezbiyen Kültürel Araştırmalar ve Dayanışma Derneği (KAOS GL) (en: Kaos Gay and Lesbian Cultural Research and Solidarity Association) have std 0.23
  \item  34 English (Australia) statements by: Royal Commission into Violence, Abuse, Neglect and Exploitation of People with Disability have std 0.22
  \item  17 Italian statements by: Uppa have std 0.21
\end{itemize}
